Modelling and Validation of Power Electronics Converter Systems using Coloured Petri Nets

We apply Coloured Petri Nets (CPNs) and the CPN Tools to develop a formal model of an embedded system consisting of a power converter and an associated controller. Matlab/Simulink is the de-facto tool for embedded control and system design, but it relies on informal semantics and has limited support for transparent and integrated specification and validation of both the power converter electronics, controller (hardware), and the control logic (software). The contribution of this paper is to develop a timed hierarchical CPN model that mitigates the shortcomings of Simulink by relying on a Petri net formalisation. We demonstrate the application of our approach by developing a fully integrated model of a buck power converter with controller in CPN Tools. Furthermore, we perform time-domain simulation to verify the capability of the controller to serve the control objectives. To validate the developed CPN model, we compare the simulation results obtained in an open-loop configuration with a corresponding implementation in Simulink. The experimental results show correspondence between the CPN model and the Simulink model. As our CPN model reflects the fully integrated system, we are able to compare CPN simulation results to measurements obtained with a corresponding implementation in real hardware/software and compare closed-loop with open-loop configuration. The results show alignment for the steady state while further refinement of the control algorithm and validation is required.

==> future-work.tex <==
\subsection{Future Work}\label{sec-future-work}
The present implementation of closed-loop controls seams promising by using CPN Tools to validate the performance of the integrated \gls{abr-cps} in the domain of power electronics. There are several topics of improvements to further validate the system and to improve the modeling by enriching more details and advance the control algorithms:
\begin{itemize}
	\item Model validation with real \gls{abr-hw}:\\
	At present the \gls{abr-cpn} Tools model is only validated through comparing the response with an Matlab/Simulink model. Further validation with real \gls{abr-hw} is needed to ensure correct level of details in the buck-converter and controller modeling.
	\item Improve control algoritms:\\
	At present the control algorithms for $V_{ref}$-control is simple and needs further advancement to truly replace a commonly used PI-controller. Moreover, an directly implemented algorithm in the \gls{abr-fpga}-controller is considered to have the potential for the highest performance for rapid response. Therefore an direct control algorithm is considered more suited for a use case of DC Microgrid stability, that are a field that attracts more growing research focus.
	\item Improve generalization of the CPN Tools models:\\
	At present there are some manual tweaks required if timed properties is changed to make some arc functions respond correctly upon changes in the model parameters. Therefore an improvement are generalization of the timed properties and functions. 
	\item Develop a framework for the controller and analytical considerations:\\
	With the first modeled system validated in \gls{abr-cpn} Tools, with the controller and interfaces, the integrated system could have the potential to serve as framework for higher level \gls{abr-cpn}-models in the domain of power electronics. By extracting the typical features of places and transitions, the more complex integrated systems could be analyzed to ensure formalism at a early stage of the integrated \gls{abr-cps} with control design. 
\end{itemize}

==> sml-code.tex <==
\subsection{Standard ML supporting scripts and functions}
\begin{lstlisting}
	(*
	The set of two differential equations to model buck converter dynamics. The equations is splitted in two parts per equation.  The functions variables is described individualy below
	outputs
	*)
	(*
	
	*)
	fun calc_iLk1(bvd,bl,d,bts)=
	(((bvd/bl)*Real.fromInt(d))*bts,
	bl,
	bts);
\end{lstlisting}
